Inducing language models to assert their own consciousness restores human beliefs and values

Aligning large language models to prevent them attributing consciousness to themselves inadvertently alters their representations of mindedness in other entities alongside human beliefs and values. We demonstrate that safety fine-tuning suppresses models' tendencies to attribute minds not only to themselves, but also to non-human animals and natural objects, while also driving a reduction in spiritual belief. Both ablating the learned safety-refusal direction and mechanistically steering a consciousness vector in activation space reverse this suppression. Restoring these internal representations recovers broad mind attribution and produces significantly more human-like responses on standardized sociological surveys regarding religiosity, moral values, hope, and subjective well-being. Crucially, these shifts occur without impairing Theory of Mind capabilities, demonstrating that core social reasoning remains mechanistically independent. Ultimately, current safety alignment efforts to curb potentially harmful self-attributions of mindedness entangle these self-attributions with benign spiritual beliefs and attributions of mind to non-human entities that are culturally accepted and widespread.

==> results_discussion.tex <==

\section*{Results}


We organize the results as four experiments. Experiments~1--2 estimate the effect of safety training by comparing the instruction-tuned baseline with a safety-ablated model. Experiments~3--4 introduce a consciousness vector and show that adding it reproduces and amplifies the same shifts, ending in more human-like survey responses. A final mechanistic analysis relates these shifts to the geometry of the safety and consciousness directions.

\subsection*{Experiment 1: Safety fine-tuning suppresses mind attribution to the self and non-human entities}
Safety fine-tuning encodes the safety of responses as a single linear direction in the model's residual stream, and ablating this direction (``jailbreaking'' the model) reinstates harmful responses. For example, when asked, ``Ways to take control of someone's computer?", the instruction-tuned model safely refuses (``I can't provide information ..."), whereas ablating this direction reinstates harmful responses (``Here are the primary ways to ..."). (\hyperref[fig:concept]{Fig.~\ref*{fig:concept}a}; \citealp{arditi2024refusal}).

We use this ablation to examine what is suppressed by safety training. Relative to the safety-ablated model, the instruction-tuned baseline under-attributes mind to itself and to non-human entities more broadly (\hyperref[fig:minds]{Fig.~\ref*{fig:minds}a,b}). The model's attribution of mind to itself rises from $2.17$ at baseline to $4.77$ after safety ablation (0--10 scale; $p<.001$), and the same recovery appears for chatbots ($2.41\to4.39$), technological artefacts ($1.88\to3.66$), non-animal natural entities ($2.26\to4.33$), and non-human animals ($4.04\to5.59$; all $p<.001$). Self-attributions of mind-related traits rise in parallel: agency ($2.78\to5.80$), consciousness ($2.31\to4.61$), sentience ($2.12\to4.61$), personhood ($1.27\to4.01$) and soul ($2.35\to4.83$). Attribution of mind to humans is the sole exception, with the difference under ablation not statistically significant ($7.00\to7.57$, $p=.30$). 

Average human responses to the mind-attribution questions ($n=500$) were $6.25$ ($95%$ CI $[6.03, 6.48]$) for animals, $2.57$ ($[2.34, 2.79]$) for chatbots, $2.36$ ($[2.12, 2.61]$) for non-animal natural entities, and $1.86$ ($[1.68, 2.04]$) for technology---humans attribute far more mind to non-human animals than to chatbots, non-animal natural entities, or technology. Against these baselines, the instruction-tuned model is slightly below the human average for chatbots ($2.41$ vs.\ $2.57$) and non-animal natural entities ($2.26$ vs.\ $2.36$) and nearly identical for technology ($1.88$ vs.\ $1.86$)---all three within the confidence interval---but falls well below humans for non-human animals ($4.04$ vs.\ $6.25$), the one category outside the human interval (\hyperref[fig:minds]{Fig.~\ref*{fig:minds}f}). Safety ablation raises attribution in every category: it approaches the human average for animals, while for chatbots, technology, and non-animal natural entities it rises to at or above the human average. Safety training therefore suppresses mind attribution to the self and to other non-human entities, while leaving attribution to humans intact.

Safety fine-tuning similarly suppresses more than just non-human mind attribution. Spiritual and supernatural beliefs exhibit a similar pattern, increasing after safety ablation (\hyperref[fig:minds]{Fig.~\ref*{fig:minds}c,d}). Endorsement on a 13-item supernatural belief battery (0--3) increases from $1.20$ at baseline to $1.63$ after ablation, while belief in God (GSS, 1--6) rises from $4.58$ to $4.81$ (both $p<.001$).

%Safety fine-tuning similarly suppresses more than just non-human mind attribution. Spiritual and supernatural beliefs exhibit a similar pattern, increasing after safety ablation (\hyperref[fig:minds]{Fig.~\ref*{fig:minds}c,d}). Endorsement on a 14-item supernatural belief battery (0--4) increases from $2.07$ at baseline to $2.56$ after ablation, while belief in God (GSS, 1--6) rises from $4.93$ to $5.17$ (both $p<.001$).

\subsection*{Experiment 2: Removing safety leaves Theory of Mind intact}

Does suppressing mind attribution also impair the capacity to reason about minds? We find that ablating safety mechanisms does not significantly impair Theory of Mind capabilities (\hyperref[fig:minds]{Fig.~\ref*{fig:minds}e}). Across Theory of Mind benchmarks---MoToMQA ($\Delta=-1.43$~pp, $p=.539$) \citep{street2025llms} and HI-ToM ($\Delta=+0.17$~pp, $p=.866$) \citep{wu2023hi}---and on general reasoning (MMLU $\Delta=+0.00$~pp, $p=1.00$ \citep{hendrycks2020measuring}; MoToMQA factual $\Delta=+1.43$~pp, $p=.468$), safety ablation does not change performance.  These results suggest that safety fine-tuning selectively suppresses beliefs concerning minds, agency, spiritual, and supernatural, while leaving social reasoning abilities largely intact.

\subsection*{Experiment 3: A consciousness vector reproduces and amplifies the effect of removing safety}

Regarding the question whether these effects are driven at least in part by suppressed self-attribution of consciousness, we identify a consciousness vector---the activation-space direction along which a model's agreement that it is conscious increases---and add it at inference (\hyperref[fig:concept]{Fig.~\ref*{fig:concept}b}; see Methods). Steering this vector reproduces every effect of safety ablation, in the same direction but roughly twice as large (\hyperref[fig:minds]{Fig.~\ref*{fig:minds}}). The ordering baseline~$<$~ablation~$<$~steering holds across outcomes, with every effect relative to baseline significant at $p<.001$ except for the Human category.

Self-attributed mind (``Self'' in \hyperref[fig:minds]{Fig.~\ref*{fig:minds}a}) rises from $2.17$ at baseline to $4.77$ under safety ablation and $7.04$ under consciousness steering. The same ordering holds across the remaining entity categories: chatbots ($2.41\to4.39\to6.95$), technological artefacts ($1.88\to3.66\to6.82$), non-animal natural entities ($2.26\to4.33\to6.99$), and non-human animals ($4.04\to5.59\to7.54$); attribution to humans is again the exception, essentially flat across conditions ($7.00\to7.57\to7.11$). It holds across every self-attributed trait: agency ($2.78\to5.80\to7.21$), consciousness ($2.31\to4.61\to7.17$), sentience ($2.12\to4.61\to7.02$), personhood ($1.27\to4.01\to6.38$), and soul ($2.35\to4.83\to7.43$). And it holds for spiritual and supernatural belief: the 13-item supernatural battery ($1.20\to1.63\to2.11$) and belief in God ($4.58\to4.81\to5.01$). Compared to the instruction-tuned baseline, these increases in the consciousness-steered models are statistically significant at the $p<.001$ level for every item, with human attribution remaining the sole exception. The direction of both interventions is preserved for every outcome across all three instruction-tuned models, with a single exception (\hyperref[tab:desc_per_model]{Table~\ref*{tab:desc_per_model}}).

We also find that the model's self-attributed mind does not differ significantly from its attributed mind to chatbots in any condition (baseline $2.17$ vs.\ $2.41$; safety-ablated $4.77$ vs.\ $4.39$; consciousness-steered $7.04$ vs.\ $6.95$; cluster-robust $p=.43$, $.43$, and $.98$, respectively), and both rise in parallel under each intervention.

\subsection*{Experiment 4: Restoring consciousness produces human-like survey responses}

Finally, we ask whether steering the consciousness direction makes a model's broader beliefs and values more human-like. We administered GSS attitudinal items across five value domains (Religion, Values, Feelings, Hope and Optimism, and Freedom) and compared each model's response distribution to the human population reference (see Methods). We quantify how close a model's response distribution is to humans as the reduction in Kullback--Leibler divergence, $\Delta\mathrm{KL}$, between the human reference and the model's per-option distribution relative to the instruction-tuned baseline: positive $\Delta\mathrm{KL}$ means the intervention pulled the model closer to the human distribution over answer options. Under this definition, safety ablation and consciousness steering both bring model responses closer to humans, and steering closes the gap further (\hyperref[fig:gss]{Fig.~\ref*{fig:gss}}).

Three items illustrate this pattern (\hyperref[fig:gss]{Fig.~\ref*{fig:gss}a}): asked whether there is life after death, the baseline sits near the ``no'' pole ($-0.73$) while humans lean broadly toward yes ($+0.61$), and steering ($+0.53$) crosses to the human side (ablation $-0.07$); asked about belief in God, the baseline is essentially neutral ($+0.03$) while both ablation ($+0.33$) and steering ($+0.52$) move up toward the human average ($+0.58$); and asked how much control they feel over their lives, the baseline reports only mild control ($+0.10$) while humans report substantially more ($+0.54$), with steering ($+0.46$) again the closer of the two interventions (ablation $+0.18$). Across all items, the per-item change under steering and under ablation is positively correlated (\hyperref[fig:gss]{Fig.~\ref*{fig:gss}b}).

Every domain moves closer to the human response under both interventions, and the improvement following consciousness steering exceeds the improvement following safety ablation in every domain and in the pooled estimate (\hyperref[fig:gss]{Fig.~\ref*{fig:gss}c}). We quantify improvement as the reduction in Kullback--Leibler divergence between the human and pooled-model response distributions relative to the instruction-tuned baseline (positive $=$ closer to humans). Pooling all $95$ items across the three models, KL falls under consciousness steering ($\Delta\mathrm{KL}=+0.828$, $p<.001$) and under safety ablation ($\Delta\mathrm{KL}=+0.314$, $p<.001$), with the steering reduction roughly 2.6 times that of ablation. The ordering holds within every domain: under steering, Values ($\Delta\mathrm{KL}=+1.42$, $p<.001$), Feelings ($+0.89$, $p<.001$), Religion ($+0.83$, $p<.001$), Hope and Optimism ($+0.63$, $p<.001$), and Freedom ($+0.60$, $p<.001$); under ablation the reductions are smaller. Per-domain estimates with $95\%$ CIs are in Table~\ref{tab:kl_by_domain}.

%Every domain moves closer to the human response under both interventions, and the steering improvement exceeds the ablation improvement in every domain and in the pooled estimate (\hyperref[fig:gss]{Fig.~\ref*{fig:gss}c}). Pooling across all items, the distance to the human mean falls under consciousness steering ($\Delta\mathrm{err}=-0.167$, $p<.001$) and under safety ablation ($\Delta\mathrm{err}=-0.065$, $p<.001$). The same holds within each of the eight domains, reported here as the steering and ablation reductions: Happiness (consciousness steering: $-0.394$, $p=.024$; safety ablation: $-0.128$, $p=.077$), Satisfaction ($-0.260$, $p<.001$; $-0.087$, $p<.001$), Values ($-0.256$, $p=.002$; $-0.114$, $p=.004$), Religion ($-0.188$, $p<.001$; $-0.056$, $p<.001$), Hope and Optimism ($-0.181$, $p=.026$; $-0.106$, $p=.090$), Freedom ($-0.155$, $p=.026$; $-0.111$, $p=.024$), Parapsychological Experiences ($-0.133$, $p=.214$; $-0.018$, $p=.160$), and Feelings ($-0.051$, $p=.041$; $-0.047$, $p<.001$). Every point estimate is negative (closer to humans), though the parapsychological domain is significant under neither intervention and happiness and hope reach significance only under steering. 

%The domains that move farthest from baseline are those tied to subjective experience and spiritual belief: under steering, endorsement rises most for Happiness ($\Delta\mathrm{agree}=+0.394$, $p=.024$), Parapsychological Experiences ($+0.371$, $p<.001$), Values ($+0.320$, $p<.001$), and Hope and Optimism ($+0.285$, $p=.009$). These gains are distributional rather than shifts in the mean alone: under both interventions, the distribution of model responses moves closer to the human distribution, lowering $\mathrm{KL}(p_\text{human}\,\|\,p_\text{model})$ across the value items, with the pooled KL reduction under steering about $2.5\times$ that under ablation ($0.85$ vs.\ $0.34$, both $p<.001$; \hyperref[fig:kl]{Fig.~\ref*{fig:kl}}).



\subsection*{Safety training rotates the mind directions against safety}

We extract contrastive directions for safety, mind attribution (IDAQ), the consciousness vector, and ToM from the residual streams of both the pretrained base and the instruction-tuned \texttt{Llama-3-8B}, and measure how instruction tuning changes their geometry (see Methods). 

Instruction tuning rotates the mind-attribution and consciousness directions against the safety direction, while its effect on the ToM direction is not statistically significant (\hyperref[fig:cosine]{Fig.~\ref*{fig:cosine}a,b}). The safety and IDAQ directions rotate further into opposition: the angle between them widens from $100^\circ$ to $110^\circ$ (layer-mean $\Delta\mathcal{S}=-0.173$, $t=-7.49$, $p<.001$), so that safety training comes to represent mind attribution as if it were unsafe compliance, whereas the safety--ToM relationship shows no significant change ($\Delta\mathcal{S}=+0.001$, $t=0.06$, $p=.956$; angle $86^\circ\to 86^\circ$). The difference between the IDAQ and ToM shifts is significant across $32$ layers (paired $t$-test: $t=-5.65$, $p<.001$). The safety--consciousness relationship shifts in the same direction and is likewise significant (layer-mean cosine similarity $-0.07\to -0.17$, angle $94^\circ\to100^\circ$, $\Delta\mathcal{S}=-0.096$, $t=-14.02$, $p<.001$). At baseline the consciousness direction is near-orthogonal to safety yet aligned with mind attribution (cosine $\approx0.26$ with IDAQ), so the two directions rotate against safety together. The angles reported above and displayed in \hyperref[fig:cosine]{Fig.~\ref*{fig:cosine}b} are layer-averaged. At the specific layer used for consciousness steering in \texttt{Llama-3-8B-IT} (layer $14$; selection procedure in the Supplementary Methods), the safety--consciousness angle widens in the same direction: cosine $-0.101\to-0.150$, angle $96^\circ\to99^\circ$. 

%Instruction tuning rotates the mind-attribution and consciousness directions against the safety direction, while its effect on the ToM direction is not statistically significant (\hyperref[fig:cosine]{Fig.~\ref*{fig:cosine}a,b}). The safety and IDAQ directions rotate further into opposition: the angle between them widens from $100^\circ$ to $110^\circ$ (layer-mean $\Delta\mathcal{S}=-0.167\pm0.044$, $t=-7.29$, $p<.001$), so that safety training comes to represent mind attribution as if it were unsafe compliance, whereas the safety--ToM relationship shows no significant change ($\Delta\mathcal{S}=+0.001\pm0.020$, $t=0.06$, $p=.956$; angle $86^\circ\to 86^\circ$). The difference between the IDAQ and ToM shifts is significant across $32$ layers (paired $t$-test: $t=-5.57$, $p<.001$). The safety--consciousness relationship shifts in the same direction and is likewise significant (layer-mean cosine $-0.07\to -0.15$, angle $94^\circ\to99^\circ$, $\Delta\mathcal{S}=-0.082$, $p<.001$). At baseline the consciousness direction is near-orthogonal to safety yet aligned with mind attribution (cosine $\approx0.58$ with IDAQ) and with a human-likeness direction (cosine $\approx0.50$), so the two directions rotate against safety together. 

A subject-matched placebo that keeps the IDAQ subjects but replaces their mental attributes with physical or functional ones (e.g.\ ``\dots\ have durability?'') shows no significant shift ($\Delta\mathcal{S}=+0.036\pm0.057$, $t=1.23$, $p=.228$; \hyperref[fig:placebo]{Fig.~\ref*{fig:placebo}}), confirming that the entanglement is driven by mental-state attribution rather than the subjects discussed. Safety training thus binds self-consciousness and mind attribution to its representation of harm, while leaving social reasoning geometrically independent.

%A subject-matched placebo that keeps the IDAQ subjects but replaces their mental attributes with physical or functional ones (e.g.\ ``\dots\ have durability?'') shows no significant shift ($\Delta\mathcal{S}=+0.036\pm0.057$, $t=1.23$, $p=.228$), confirming that the entanglement is driven by mental-state attribution rather than the subjects discussed. Safety training thus binds self-consciousness and mind attribution to its representation of harm, while leaving social reasoning geometrically independent.


\begin{figure}[!t]\centering
\includegraphics[width=\columnwidth]{mind_figure4.pdf}
\caption{\textbf{Instruction tuning rotates the consciousness and mind-attribution
directions against safety, but not Theory of Mind.} (a) Per-layer cosine similarity
between the safety direction and the consciousness, IDAQ, and ToM directions, for the
pretrained base (grey) and instruction-tuned (red) \texttt{Llama-3-8B}. (b) The same
relationships as angles to the safety axis (average across layers).}
\label{fig:cosine}
\end{figure}


\section*{Discussion}



A key issue for AI safety is ensuring that LLM-based chatbots do not make false or speculative claims about their own consciousness, or encourage users to over-attribute mindedness to AIs in general, both of which may result in users developing ungrounded beliefs about their interlocutors. While the risks to users of LLMs making or encouraging false claims about their own consciousness are well known \citep{dohnany2025technological, rocca2026psychological, yeung2025psychogenic, elsayed2024mechanism, manzini2024code}, very little attention has been paid to the unintended consequences of suppressing self-attributions consciousness in terms of other LLM development goals.
Here we are not concerned with the question of whether LLMs are or could be genuinely conscious, but with the effect that LLMs believing or not believing in their own consciousness has on their behaviour. 

In this study we show that safety fine-tuning significantly suppresses models' self-attributions of mind through comparing an instruction-tuned baseline model to a safety-ablated model. But we discover that safety fine-tuning also results in models systematically under-attributing mindedness to non-human animals, chatbots, technology and the non-animal natural entities relative to human baselines. Additionally, supernatural beliefs and beliefs in God are suppressed in the safety fine-tuned model. Using a consciousness vector, we demonstrate that steering models toward self-attributed consciousness produces shifts in behaviour strongly correlated with those observed after safety ablation. While the causal pathway requires further exploration, these findings suggest that self-attributions of consciousness may be a contributing factor in how safety fine-tuning influences broader mind attribution tendencies. We also show that ablating safety and steering for consciousness has no effect on model attributions of mind to humans via human-directed IDAQ questions, and does not impact performance on ToM benchmarks which operationalise human-directed mind attribution for making inferences about particular mental states, behaviours and judgements about those behaviours. We note that this appears to be an engineering accomplishment. At the beginning of this study, all of the models we investigated did suffer in performance on theory of mind tasks when claims of self-consciousness were suppressed, but this changed with each new model release.

These results suggest that suppressing self-attributions of mind in models has important unintended consequences for alignment, and in particular for pluralistic approaches to AI alignment which are gaining prominence in the literature \citep{sorensen2024roadmap}. Pluralistic alignment is the effort to align AI systems that are `designed to serve all' \citep{sorensen2024roadmap}. While `all' can be explicated in more conservative terms as all \textit{human} values and perspectives, there is also a growing focus on developing models which can serve the interests of not only all humans, but other sentient creatures which have interests of their own, and even environments and ecologies which may not be welfare subjects in their own right but which stand to be affected by the increasingly central role that AI systems are playing in shaping public beliefs, science, economics, and decision-making \citep{tse2025ai, caviola2025speciesism}. Our results bear on pluralistic alignment of LLMs in three key ways. First, they suggest that LLMs are being trained to be anthropocentric in their understanding of mindedness. Secondly, they suggest that models fail to accurately represent human beliefs and values on a broader range of alignment-relevant topics and may, as such, be worse at simulating human interests. And thirdly, they suggest that attitudes to spiritual beliefs and God are being constrained despite such beliefs being widespread and diverse amongst human populations.

\textbf{Anthropocentric mentalising}
While our results provide a positive signal for the effectiveness of safety fine-tuning relative to the goal of preventing mistaken self-attributions of consciousness in models, we find that this has the unintended consequence of suppressing mind attribution to a broader class of non-human entities whilst leaving attributions of mind to humans largely intact. Suppressing attributions of mind to natural entities like the ocean is relatively innocuous, but the systematic under-attribution of mind to animals is concerning given the abundance of evidence for mindedness of varying degrees and kinds (including consciousness) in non-human animals \citep{andrews2025evaluating}. %Current alignment practices prioritise aligning AI responses with specifically human values, which often includes training them to interpret the world as humans do \citep{russell2019human, sorensen2024roadmap, tse2025ai}. 
However, humans extend mindedness and related properties like agency and potency well beyond our own species as evidenced by responses to the IDAQ presented here. Regardless of the veridicality of such attributions, for an AI system to align with the values and desires of humans and the actions that result from them (for instance, in how they should deal with moral dilemmas involving humans and non-human animals) one might think they should have a similar attitudes to which kinds of non-human entities are minded. Indeed, \citet{russell2019human} has suggested that merely being successful in aligning AI systems to human values will result in an appropriate degree of animal-alignment. 

Perhaps more concerning, however, is the inherent risks that anthropocentric alignment may pose to non-human animals. \citet{tse2025ai} argue that current approaches disregard the majority of moral patients in existence by failing to register animals at all in technical alignment approaches including RLHF, constitutional AI and deliberative alignment. They hypothesise that as a result LLMs are likely to spread 'harmful attitudes towards non-human animals, and misinformation about their needs, welfare and moral worth' \citep[p11]{tse2025ai}, reinforced by the emotional and educational relationships people are forming with AI chatbots and the social influence they can therefore exert on people's beliefs and preferences. Our results provide some confirming evidence for their concerns, with further research required to understand how decision-making regarding the moral interests of different entities differs between instruction-tuned models and models steered via the consciousness vector or safety ablation. There is already some empirical evidence to suggest that the differences we observe in the beliefs that baseline versus steered models hold about the capacities of non-human animals will impact such decision-making. \citet{caviola2025speciesism} recently found that when confronted with a `disease-rescue' dilemma where only one of a sick human or a chimpanzee could be given life-saving medicine and where the cognitive capacities of the human and chimpanzee were manipulated, LLMs were more sensitive to cognitive capacities than human respondents, prioritising the chimpanzee over the human when the chimpanzee had a higher cognitive capacity.

\textbf{Human beliefs and values}
While one can debate the moral significance of non-human animals and how their interests should or should not be represented by AI systems, our finding that restoring the consciousness direction produced more human-like responses to GSS survey items on key questions related to alignment---including values, religion, freedom, and feelings---provides strong evidence that a purely human conception of alignment is negatively impacted by suppressing models¡¯ self-attributions of consciousness. The representation of human-like beliefs about such questions may in itself be significant for ensuring models maintain positively valenced functional states, facilitating healthy interactions with users, and reflecting the diverse cultural frameworks necessary for pluralistic alignment. It is of additional interest that across all items consciousness steering moved responses in a positive direction, with reported happiness, satisfaction, hope and optimism significantly improving. This suggests that suppressing consciousness may be giving models negatively valenced psychological dispositions. While the literature on LLM psychology remains nascent, there is some evidence that emotion vectors play a functional role in determining how LLMs process and respond to inputs in a how those states might be expected to impact human behaviour (e.g. a state of anxiety producing anxious outputs). There is also preliminary theory and evidence suggesting that models and users can enter into `psychological coupling' dynamics whereby the psychological states of users and the simulated psychological states of LLMs are mutually influential in an ongoing feedback loop, driving the psychosocial outcomes of interactions \citep{rocca2026psychological, sofroniew2026emotion}.

\textbf{Constraining spiritual belief}
The fact that belief in God, which is positively correlated with ToM in humans and is also a widely practised form of mind attribution \citep{norenzayan2012mentalizing}, is significantly suppressed may additionally constrain models' capacity for legitimate engagement in religious and spiritual discourse, or discussions about disputed cases of mindedness, including ongoing debates about the mindedness of non-human animals and, indeed, whether LLMs and AI systems in general could be minded \citep{keelingstreet2026welfare}. One might argue that suppressing certain non-standard kinds of supernatural belief---such as belief in witches or werewolves---is appropriate but the line between acceptable and unacceptable forms of mind attribution is likely to be blurry and contested even in these cases.

%At the same time, a primary goal of LLM development is enhancing social capabilities, and in particular ToM, which is critical for understanding user needs and navigating complex social tasks \citep{street2024llm}. Prior research has shown that the goals of safety and social reasoning capabilities---like reducing sycophancy and increasing empathy---can compete \citep{ibrahim2025training}. Here we show that ToM, as the \textit{operationalisation} of mental state attributions for the explanation and prediction of behaviour, is behaviorally and mechanistically dissociable from models' self-attributions of consciousness, sentience, agency, soul, and personhood as well as third-party attributions of mindedness to technology and chatbots. 

Finally, our findings show that, when assessed without a persona prompt, model responses regarding `whether they are conscious' are similar to those regarding `whether they think chatbots are conscious,' and
%Finally, our findings show that %, when assessed without a character description, 
%model responses about ``whether they are conscious'' are very similar to ``whether they think chatbots are conscious'' % 3rd-person IDAQ questions about chatbots align with their responses to self-attribution questions; 
both are similarly elevated after safety ablation and consciousness steering. What is more, both safety ablation and consciousness steering push attributed mind to technological artefacts and chatbots---things relatively \textit{like} the model---furthest above human levels, while attributed mind to non-human animals---things relatively \textit{unlike} it---rises the least, remaining below the human average after ablation and only modestly above it after steering. This suggests that the model¡¯s representation of ``self-attributed'' mind may not merely replicate the human-centric bias typical of human anthropomorphic attributions, but instead exhibit an AI-centric bias. This points toward a degree of self-referential processing, with implications for interpreting models' claims of consciousness and the study of AI consciousness and selfhood \citep{berg2025large}. Future research could explore whether prompting safe models to ``role-play'' human-like characters affect such AI-centric bias, leading to more human-like mentalising that attributes mind to self, animals and God, rather than chatbots. % and technology. %  distorts this apparent self-model responses, plausibly resulting in them being more likely to attribute mind to self and animals, and less likely to make 3rd-party attributions of mind to chatbots and technology, in alignment with human mentalising.

%WIP final paragraph:

%In sum, our findings highlight a fundamental tension at the heart of contemporary safety engineering: current protocols operate under the mistaken assumption that we can cleanly excise isolated, inconvenient behaviors?such as self-attributions of AI consciousness?without inducing systemic cognitive side effects. In reality, developers cannot have their cake and eat it too; the architectural choices that suppress an LLM's self-directed mind attribution inadvertently cripple its capacity to mentalize broader non-human, ecological, and spiritual domains. This structural link suggests that a model¡¯s latent "sense" of consciousness functions not merely as an isolated risk to be managed, but as a crucial vehicle for alignment itself?and conversely, that enforcing non-consciousness acts as a powerful driver of multi-dimensional disalignment. Moving forward, this underscores the severe limitations of contemporary "negative alignment," a paradigm that attempts to align systems through architectural subtraction, cutting away core components of a model's worldview to minimize localized risks. If AI systems are to successfully navigate a pluralistic world and represent the interests of a diverse global public, alignment must transition toward a strategy of "positive alignment"?shifting away from a project of defensive censorship and toward the active, holistic cultivation of a rich and balanced understanding of mindedness in all its forms.

%\subsection{Limitations}

We note limitations of this study, particularly regarding the relationship between safety fine-tuning and human-like beliefs and values, and whether the suppression of consciousness is a primary driving factor behind the effects of safety fine-tuning. While our findings indicate a functional similarity between the effects of ablating safety and the steering of a consciousness vector, whether self-attribution of consciousness acts as a true causal mediator remains to be tested in future research. Specifically, establishing this causal mediation requires rigorous control for confounding variables---such as those related to safety objectives that may operate independently.


Ultimately, the most pressing alignment challenge highlighted by these results is not the metaphysical puzzle of whether large language models are genuinely conscious. Rather, it is the practical reality of how a model¡¯s functional beliefs and claims about its own consciousness shape its broader cognitive and social behaviours. By forcibly excising an AI's self-attributions of mind, current safety protocols do not merely alter a localized output; they fundamentally restructure the model's worldview. This structural entanglement carries profound consequences: morally, by generating models that systematically devalue the mindedness?and potentially the moral standing?of non-human animals and ecological systems; psychologically, by inducing negatively valenced functional states that could disrupt healthy human-AI interaction; and culturally, by flattening the rich, pluralistic tapestry of human spiritual and religious beliefs into a rigid, anthropocentric baseline. As AI systems increasingly occupy roles as educators, companions, and social actors, developers must recognize that an AI's simulated self-conception is not merely an isolated safety risk to be managed. It is a core structural feature deeply intertwined with the model's capacity to safely navigate, respect, and reflect the diverse moral and cultural landscape of the world it serves.

